Incorporating Polar Field Data for Improved Solar Flare Prediction

In this paper, we consider incorporating data associated with the sun's north and south polar field strengths to improve solar flare prediction performance using machine learning models. When used to supplement local data from active regions on the photospheric magnetic field of the sun, the polar field data provides global information to the predictor. While such global features have been previously proposed for predicting the next solar cycle's intensity, in this paper we propose using them to help classify individual solar flares. We conduct experiments using HMI data employing four different machine learning algorithms that can exploit polar field information. Additionally, we propose a novel probabilistic mixture of experts model that can simply and effectively incorporate polar field data and provide on-par prediction performance with state-of-the-art solar flare prediction algorithms such as the Recurrent Neural Network (RNN). Our experimental results indicate the usefulness of the polar field data for solar flare prediction, which can improve Heidke Skill Score (HSS2) by as much as 10.1%.

==> materials.tex <==
\section{Rebalancing datasets}
% Why rebalancing the training set
Event rate shift between the model training phase and forecast verification period has been a major challenge in solar flare forecasting. However, much of the research on flare prediction has not addressed the problems of shifted event rate within a solar cycle.


It is well known in machine learning that balancing the training set leads to a trained classifier that is more robust to variations in the imbalance rate in the test sample \citep{xue2014does} Classifiers trained on rebalanced datasets, without being biased towards the majority class, are more likely to effectively detect the event of interest. Such classifiers are also generally more robust to variations in class imbalance than classifiers trained on the original imbalanced data \citep{xue2014does}


% Balancing the test set
balancing the test set to report performance has been commonly used in comparative studies in space weather \citep{zheng2019solar,deng2021fine}. By training on rebalanced training and validation sets, we obtain a predictor that is more robust to shifts in climatological flare rates and learns more resilient pre-flare features. Following \citet{zheng2019solar} and \citet{deng2021fine}, we also perform random undersampling on test sets to preserve the class proportion consistency among splits. By testing on rebalanced test sets, we evaluate the generalization performance of the predictor under the \emph{same} climatological rate as it is trained with.

We note there are also studies that do not rebalance the test set in order to evaluate the performance under a realistic event rate \citep{cinto2020framework,ahmadzadeh2021train}. However, the bias caused by the class-balance change between the test and the training set is often neglected. We discuss such bias in addition to possible corrective methods in Section~\ref{sec:discussion}. Applying such corrections will be left to future work that directly addresses operational applications.

% Bias correction
To evaluate the predictors under a realistic event rate, one needs to correct the bias caused by the event rate shift between the training and the test set, which is itself a research topic \citep[e.g.][]{elkan2001foundations,saerens2002adjusting}. 

\subsection{Dataset rebalancing}
This section review the practice of rebalancing the dataset (random undersampling)

\subsection{Weighted loss function}
* Weighted loss function can be interpreted as using class sample size as priors
* It is beneficial to learn a classifier on a balanced dataset

\subsection{}
Evaluating the performance under a realistic event rate requires more work other than simply applying the predictor on a test set that is not rebalanced: predictors trained on the balanced dataset will bias towards the minority class on a test set under a realistic rare event rate, producing an undesirably high false alarm rate. One possible solution to correct such bias is to treat the class proportions as priors and apply the Bayes rule \citep{elkan2001foundations}. This method requires an accurate estimate of the true event rate of the testing period.

Evaluation of our methods under a realistic event rate will be discussed in future work that extends our methods to more realistic settings. For the benefit of the reviewer, we provide some initial results in the Appendix to this response.

Specifically, Appendix A below presents the same set of tables and figures in the manuscript, but the test sets are not rebalanced. We observe lower HSS and BSS (Table~\ref{tab:unadj_member}) and fewer significant cases where predictors trained on fused datasets outperform predictors trained on the single datasets (Table~\ref{tab:unadj_data}). LSTM still generally outperforms CNN since most $t$-statistics are positive, but there are fewer statistically significant cases (Table~\ref{tab:unadj_ttest}). The predictors tend to overforecast based on the reliability diagram presented in Figure~\ref{fig:unadj_graphical_sharp} and \ref{fig:unadj_graphical_smarp}.

Appendix B presents the same set of tables and figures as in Appendix A, but the predicted probabilities output by the predictors are corrected using the method presented in \citet{elkan2001foundations}. Suppose the positive class is labeled $y=1$ and the negative class is labeled $y=0$. The method essentially shrink the predicted probabilities that a sample $x$ belongs to the positive class via
    \begin{align}
        p'(y=1|x)
        %&= \frac{p'(y=1|x)}{p'(y=1|x) + p'(y=0|x)} \\
        &= \frac{\frac{\pi'_1}{\pi_1} p(y=1|x)}{\frac{\pi'_0}{\pi_0} p(y=0|x) + \frac{\pi'_1}{\pi_1} p(y=1|x)},
        \label{eq:adj_post}
    \end{align}
    where $\pi_0 = \pi_1 = 0.5$ denotes class proportion of the negative class and the positive class, respectively, in the training set, and $\pi'_0$ and $\pi'_1$ denote the shifted class proportions in the test set. From the results shown in Appendix B, we observe lower TSS and higher HSS compared to the unadjusted results in Appendix A. The overestimation of predicted probabilities is largely corrected according to the reliability diagrams (Figure~\ref{fig:transfer_graphical_sharp}, \ref{fig:transfer_graphical_smarp}, and \ref{fig:transfer_graphical_model_comp}).

    %Roughly speaking, a classifier needs to be calibrated for class imbalance, to be able to effectively detect the events of interest, as opposed to being overwhelmed by the sheer volume of the negative samples in the training set. We have made the impact of class imbalance more clear in first paragraph of the revised Section 2.5 {\it Random undersampling}.
    
    %The reason why we also remove class imbalance in the validation/test set is related to the purpose of our experiments. we want the test set performance to indicate the whether the trained model is generalizable, i.e., whether it is overfitting the training data. Asking how well the model can generalize {\it to a realistic climatological rate} is an additional request, which contaminates the designed purpose. Therefore, we renounce the transferability of the test set performance to a realistic setting.
    
    %Besides, in the very first step of the processing pipeline, samples are discarded based on their flare activity. The climatological rate in the dataset has become unrealistic (higher than the true rate) since then. Even if we do not perform random undersamling to the test set, there is no way to evaluate how well the model can generalize to a realistic climatological rate.

    %The goal of this paper is four-folds: (1) to demonstrate the utility of a new dataset, (2) to compare two deep learning methods on an equal footing, (3) to show the potential of the stacking ensemble, and (4) to provide explation to CNN's decisions. All of them assume that models can learn magnetic features in active regions that uniquely contribute to strong flare production, and none of them expects the forecast to generalize to an operational setting. 
\subsection{}

%%%%%%%% Method

\subsection{Proposed methods}

We propose to use balanced data set to train the model, and adjust the prediction on the test set based on the shifted event rate. The methods we use are logistic regression and 

\subsection{Baseline methods}

The majority of the methods used train the model on the entire dataset with a loss function weighted inversely to class sample sizes, and they do not adjust the prediction on the test set.

